Verifying Relational Properties using Trace Logic

We present a logical framework for the verification of relational properties in imperative programs. Our work is motivated by relational properties which come from security applications and often require reasoning about formulas with quantifier-alternations. Our framework reduces verification of relational properties of imperative programs to a validity problem into trace logic, an expressive instance of first-order predicate logic. Trace logic draws its expressiveness from its syntax, which allows expressing properties over computation traces. Its axiomatization supports fine-grained reasoning about intermediate steps in program execution, notably loop iterations. We present an algorithm to encode the semantics of programs as well as their relational properties in trace logic, and then show how first-order theorem proving can be used to reason about the resulting trace logic formulas. Our work is implemented in the tool Rapid and evaluated with examples coming from the security field.

==> lemmas.tex <==

\subsection{Trace Lemmas}
\newcommand*{\anddot}{%
	\mathclose{}%
	\nonscript\mskip.5\thinmuskip
	\boldsymbol{.}%
	\;%
	\mathopen{}%
}

Let $X$ denote the set of program variables $x(l) \in X$ such that $x(l)$ denotes the symbolic value of program variable $x$ at program location $l$.
\newline Let $I$ denote the set of iterators $it \in I$. Let $n$ denote the last and $\texttt{zero}$ denote the first iteration of a loop. Let $\texttt{succ}(it)$ denote the next iteration after $it$ and let $\texttt{lastIt}(tr)$ denote the last iteration of a loop where the loop condition holds.
Each program variable $x(l)$ within a loop takes as argument the iteration $it$, such that $x(l(it))$ is the value of the variable $x$ at location $l$ in iteration $it$. 
\newline\noindent Let $T = \{t_1, t_2\}$ denote the set of program traces and let $x(l(it), t)$ be the variable $x$ at location $l$ in iteration $it$ of trace $t$. Let further $ P(it) := x(l(it), t_1) = x(l(it), t_2) $.

\subsection*{At least one iteration}
Let $C(l(\texttt{zero})))$ denote the value of the loop condition at location $l$ at iteration $\texttt{zero}$. If the loop condition holds, we know there must at least exist one iteration of the loop. 

\[ \forall  tr_{\in T}. \: \Big( C(l(\texttt{zero})) \Rightarrow \exists it_{\in I} \anddot \texttt{succ}(it) = \texttt{lastIt}(tr) \Big)\]
	
\subsection*{Injectivity of iterations}
\begin{gather*}
	\forall it_{\in I} \anddot \\ \bigg( \big( \texttt{succ}(it) < n \wedge x(l(\texttt{succ}(it))) = x(l(it)) +1 \big) \Rightarrow \\
	\forall it_{1 \in I}, it_{2 \in I} \anddot \big(x(l(it_1)) = x(l(it_2)) \Rightarrow it_1 = it_2\big) \bigg)
\end{gather*}

\subsection*{Synchronization of orderings - incrementing loop counters}
\begin{gather*}
\forall  tr_{\in T}, it_{1 \in I}, it_{2 \in I} \anddot it_1 < it_2 \Rightarrow x(l(it_1), tr) <  x(l(it_2), tr)
\end{gather*}

\subsection*{Same number of iterations over two traces}

\begin{gather*}
\Big(\big(\forall  it_{\in I} \anddot it < \texttt{lastIt}(t_2) \Rightarrow i(l(it), t_1) < a.length(t_1) \big) \\
\wedge\: \big( i(l(\texttt{lastIt}(t_2)), t_1) \geq a.length(t_1) \big) \Big) \\
\Rightarrow \texttt{lastIt}(t_1) = \texttt{lastIt}(t_2)
\end{gather*}

\subsection*{Induction on $=$ over traces}
\begin{gather*}
\forall  tr_{\in T} \anddot  \\
\Big(\big(\forall  it_{\in I} \anddot it < \texttt{lastIt}(tr) \Rightarrow x(l(it), tr) = x(l(\texttt{succ}(it)), tr)\big) \\
\Rightarrow  x(l(\texttt{zero}), tr) = x(l(\texttt{lastIt}(tr)), tr)
\Big)
\end{gather*}

\subsection*{Intermediate value lemma with traces}
\begin{gather*}
\forall  tr_{\in T}, v_{\in Int} \anddot \\  \Big((x(l(\texttt{zero}), tr) \leq v \:\wedge\:  v < x(l(\texttt{lastIt}(tr)), tr))   \\
\Rightarrow \exists it_{\in I} \anddot (v = x(l(it), tr) \:\wedge\: it < \texttt{lastIt}(tr) )\Big )
\end{gather*}

\subsection*{Same values over two traces}
\begin{gather*}
\big(  x(l(\texttt{zero}), t_2) = x(l(\texttt{zero}), t_2) \:\wedge \\
( \forall it_{\in I}\anddot x(l(it), t_1) = x(l(it), t_2) \Rightarrow x(l(\texttt{succ}(it)), t_2) = x(l(\texttt{succ}(it)), t_2)   )\big) \\
\Rightarrow \forall it_{\in I}\anddot x(l(it), t_1) = x(l(it), t_2)
\end{gather*}

\subsection*{Equality preservation over traces from iteration 0 to k}
\begin{gather*}
\forall it_{R \in I} \anddot  \\ \Big(\big(P(\texttt{zero})  \:\wedge \: \forall it_{\in I} \anddot ((it < it_R \:\wedge \:
P(it)) \Rightarrow P(\texttt{succ}(it))) \big)  \\
\Rightarrow P(it_R)\Big)
\end{gather*}

\subsection*{Equality preservation over traces from iteration k to n}
\begin{gather*}
\forall it_{L \in I}\anddot  \\ \Big(\big(P(it_L)  \:\wedge \: \forall it_{\in I} \anddot ((it_L \leq it \:\wedge\: P(it)) \Rightarrow P(\texttt{succ}(it)))  \big)  \\
\Rightarrow P(n) \Big)
\end{gather*}

\end{document}

